Super Exponentials in Linear Logic

Following the idea of Subexponential Linear Logic and Stratified Bounded Linear Logic, we propose a new parameterized version of Linear Logic which subsumes other systems like ELL, LLL or SLL, by including variants of the exponential rules. We call this system Superexponential Linear Logic (superLL). Assuming some appropriate constraints on the parameters of superLL, we give a generic proof of cut elimination. This implies that each variant of Linear Logic which appears as a valid instance of superLL also satisfies cut elimination.

==> eptcsdata.tex <==
\providecommand{\firstpage}{50}
\providecommand{\publicationstatus}{U. Dal Lago and V. de Paiva (Eds.) Second Joint International\\ Workshop on Linearity \& Trends in Linear Logic and Applications.\\
EPTCS 353, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.353.3}{10.4204/EPTCS.353.3}}

